Did the Musk Takeover Boost Contentious Actors on Twitter?

Twitter has been accused of a liberal bias in its account verification and content moderation policies. Elon Musk pledged, after his acquisition of the company, to promote free speech on the platform by overhauling verification and moderation policies. These events sparked fears of a rise in influence of contentious actors -- notably from the political right. In this article, I use a publicly released list of 138k Twitter accounts that purchased blue check verification during the open window of November 9-November 11, 2022. I retrieve 4.9m tweets from a sample of politically contentious accounts. I then compare engagement on contentious user posts before and after the Musk acquisition. I find that the period following the Musk acquisition saw a substantive increase in post engagement. There is no additional increase following blue tick verification. I explain the findings with reference to an increase in activity by a newly sympathetic user base.

==> src/chapters/cuttings.tex <==
After a series of failed attempts at opening up the verification process to a wider audience, Twitter built verification requests into the platform architecture for a relaunch in 2021 \citep{twitter_relaunching_2021}.\footnote{See: \url{https://web.archive.org/web/20160802092920/https://support.twitter.com/articles/20174631} for details of previous launch.}

The politicization of the verification process has long hampered its success. In 2017, its verification service was paused after a furore following the verification of far-right figure, Jason Kessler. Following the acquisition of Twitter by Elon Musk in October, 2022, he pledged to overhaul both content moderation and verification procedures. In a tweet posted on November 1, Musk wrote that "Twitter’s current lords \& peasants system for who has or doesn’t have a blue checkmark is bullshit" and vowed to introduce a paid "Twitter Blue" verification service to take its place.\footnote{See: \url{https://twitter.com/elonmusk/status/1587498907336118274}.}

\begin{figure}
    \includegraphics[width=0.5\textheight]{src/figures/musktweet.png}
    \caption{Tweet by Elon Musk posted on Nov 1, 2022}
    \label{fig:musktweet}
\end{figure}

For the second dataset, I take a random sample of user names pulled from the entire list of 138k accounts. I refer to this as my \textbf{\textit{general}} sample.  In total, it was possible to gather data for 943 general accounts, giving $\sim$1.3m tweets. 

Given known concerns of the algorithmic amplification of particular political actors \citep{huszar_algorithmic_2022}, the use of both samples provides some guard against concerns that any engagement uptick might result from algorithm changes rather than blue-tick verification.


Musk's apparent free speech fundamentalism, alongside the opening up of blue tick verification, therefore raises urgent questions about the continued reputation of Twitter as the 'digital public square.'

%history and context of blue tick as well as confusion around meaning
The blue tick was first introduced to Twitter in 2009 to combat a spate of imposters and parody accounts \citep{kanalley_why_2013, cashmore_twitter_2009}. The politicization of the verification process has long hampered its success. In 2017, its verification service was paused after a furore following the verification of far-right figure, Jason Kessler. Following the

In the aftermath of the purchase, Twitter was flooded with a large number of users testing the limits of platform moderation polifices by posting racial slurs and other hateful speech \citep{network_contagion_research_institute_ncri_io_evidence_2022}


Verification is central to the study of online communication and misinformation for its role in signalling account authenticity and credibility as well as the increased visibility enjoyed by verified users online. Moderation is central to curbing the spread of harmful and hateful forms of information spreading online. 
